Deep Learning-based Code Completion: On the Impact on Performance of Contextual Information

Code completion aims at speeding up code writing by recommending to developers the next tokens they are likely to type. Deep Learning (DL) models pushed the boundaries of code completion by redefining what these coding assistants can do: We moved from predicting few code tokens to automatically generating entire functions. One important factor impacting the performance of DL-based code completion techniques is the context provided as input. With "context" we refer to what the model knows about the code to complete. In a simple scenario, the DL model might be fed with a partially implemented function to complete. In this case, the context is represented by the incomplete function and, based on it, the model must generate a prediction. It is however possible to expand such a context to include additional information, like the whole source code file containing the function to complete, which could be useful to boost the prediction performance. In this work, we present an empirical study investigating how the performance of a DL-based code completion technique is affected by different contexts. We experiment with 8 types of contexts and their combinations. These contexts include: (i) coding contexts, featuring information extracted from the code base in which the code completion is invoked (e.g., code components structurally related to the one to "complete"); (ii) process context, with information aimed at depicting the current status of the project in which a code completion task is triggered (e.g., a textual representation of open issues relevant for the code to complete); and (iii) developer contexts, capturing information about the developer invoking the code completion (e.g., the APIs frequently used). Our results show that additional contextual information can benefit the performance of DL-based code completion, with relative improvements up to +22% in terms of correct predictions.

==> tables/comparison_baseline_long.tex <==
% !TEX root = ../main.tex

% Design tables. 


\begin{table}[ht]
	\centering
	\caption{Complementarity analysis: between the correct predictions (CP) generated by the \emph{baseline} and by the models exploiting different contextual information.}
	\scriptsize
	\label{tab:complementarity}
	\begin{adjustbox}{width=\columnwidth,center}

	\begin{tabular}{lrrr}
	\toprule
	\multirow{2}{*}{\bf Context} &  {\bf \%CP}  &  {\bf \%CP Only} &  {\bf \%CP Only}\\
	 & {\bf  Shared}  & {\bf Baseline} & {\bf Context}\\\midrule
	                     Method Calls                      & 78.12\% & 8.29\% & 13.59\% \\
	                     Class Signatures                         & 79.03\% & 9.4\% &11.57\% \\
	                     Most Similar Method         & 73.8\% & 10.22\% & 15.98\% \\
	                      Issue Title                      & 82.85\% & 7.48\% & 9.67\% \\
	                      Issue Body                         & 82.74\% & 8.35\% & 8.91\% \\	                     
	                      Frequent Invocations                         & 80.45\% & 8.01\% & 11.54\%\\
	                      Most Similar Statements                      & 79.79\% & 9.49\% & 10.72\%\\\midrule

	                     Most Similar Method + Class Signatures   & 72.62\% & 10.78\% & 16.6\% \\
	                     Method Calls + Class Signatures       & 75.73\% & 8.75\% &15.52\% \\
	                     Most Similar Method + Method Calls& 72.52\% & 10\% & 17.48\% \\	                    
	                     Most Similar Method + Method Calls + Class Signatures        & 71.72\% & 9.75\% & 18.53\% \\
	                      Issue Title + Issue Body        & 81.68\% & 8.24\% & 10.08\% \\	                      
	                      Frequent Invocations + Most Similar Statements        & 78.01\% & 10.15\% & 11.84\% \\\midrule	 
	                      Best Code + Best Process                      & 72.72\% & 9.39\% & 17.89\% \\
	                      Best Code + Best Developer		& 73.27\% & 9.31\% & 17.42\\
	                      Best Developer + Best Process       & 80.37\% & 8.48\% & 11.15\% \\
	                      Best Code+ Best Developer + Best Process        & 71.46\% & 10.32\% & 18.22\% \\

\bottomrule
\end{tabular}
\end{adjustbox}
\end{table}
	














==> tables/datasets_table_long.tex <==
% !TEX root = ../main.tex

% Design tables. 	
	
\begin{table}[ht]
	\centering
	\caption{Fine-tuning Datasets.}
	\scriptsize
	\label{tab:datasets}
	\begin{adjustbox}{width=\columnwidth,center}
	\begin{tabular}{lrrr}
	\toprule
	\multirow{2}{*}{{\bf Context}}  & \multicolumn{3}{c}{\bf Instances Length}\\ \cline{2-4}
	& {\bf Mean} & {\bf Median} & {\bf St. Dev.}\\\midrule
Baseline  & 243 & 205 & 166\\
Method Calls  & 380 & 326 & 253\\
Class Signatures  & 733 & 481 & 1,128\\
Most Similar Method  & 447 & 384 & 296\\
Issue Title  & 260 & 222 & 167\\
Issue Body  & 550 & 361 & 1,429\\
Frequent Invocations  & 467 & 418 & 252\\
Most Similar Statements  & 517 & 445 & 2,355\\\midrule

Most Similar Method + Class Signatures  & 941 & 693 & 1,169\\
Method Calls + Class Signatures  & 871 & 621 & 1,153\\
Most Similar Method + Method Calls  & 584 & 507 & 374\\
Most Similar Method + Method Calls + Class Signatures  & 1,079 & 829 & 1,200\\
Issue Title + Issue Body  & 567 & 378 & 1,430\\
Frequent Invocations + Most Similar Statements   & 741 & 647 & 2,365\\\midrule
Best Code + Best Process  & 601 & 525 & 376\\
Best Code + Best Developer  & 808 & 735 & 423\\
Best Developer + Best Process  & 484 & 435 & 254\\
Best Code+ Best Developer + Best Process  & 825 & 753 & 425\\
%Limited 3 Lines  & 56 & 53 & 25\\
%Limited 2 Lines  & 72 & 69 & 32\\
	                      

\bottomrule
\end{tabular}
\end{adjustbox}
\end{table}





==> tables/performance_long.tex <==
% !TEX root = ../main.tex

% Design tables. 

\begin{table}[ht]
	\centering
	\caption{Percentage of correct predictions.}
	\scriptsize
	\label{tab:performance}
	\begin{adjustbox}{width=\columnwidth,center}
	\begin{tabular}{llr}
	\toprule
	{\bf Context} &  \multirow{2}{*}{\bf Context}  & {\bf \%Correct}\\ 
	{\bf Type} &  & {\bf Prediction}\\\midrule
	     None                 & Baseline                             & 30.58\% \\\midrule
	                              & Method Calls                      & 32.46\% \\
	                     & Class Signatures                         & 31.33\% \\
	                      &  Most Similar Method         & 32.68\% \\
	     Single                  & Issue Title                      & 31.32\% \\
	          		& Issue Body                         & 30.77\% \\
	          & Frequent Invocations                         & 31.80\% \\        
	             	         &  Most Similar Statements                      & 31.00\% \\\midrule 
	                     
\multirow{6}{*}{Within-family} 	         & Most Similar Method + Class Signatures                         & 32.72\% \\
	                  & Method Calls + Class Signatures                     & 33.03\% \\
	                      &  Most Similar Method + Method Calls & 33.35\% \\
	                      &  Most Similar Method + Method Calls + Class Signatures        & 33.88\% \\
		                      &  Issue Title + Issue Body        & 31.20\% \\	                      
	                      &   Frequent Invocations + Most Similar Statements        & 31.17\% \\\midrule	 
	  \multirow{4}{*}{Cross-family}          & Best Code + Best Process                      & 33.75\% \\
	            & Best Code + Best Developer& 33.58\% \\
	                      &  Best Developer + Best Process        & 31.50\% \\
	                      &  Best Code+ Best Developer + Best Process        & 33.54\% \\
\bottomrule
\end{tabular}
\end{adjustbox}
\end{table}






